Coupling of IGA and Peridynamics for Air-Blast Fluid-Structure Interaction Using an Immersed Approach

We present a novel formulation based on an immersed coupling of Isogeometric Analysis (IGA) and Peridynamics (PD) for the simulation of fluid-structure interaction (FSI) phenomena for air blast. We aim to develop a practical computational framework that is capable of capturing the mechanics of air blast coupled to solids and structures that undergo large, inelastic deformations with extreme damage and fragmentation. An immersed technique is used, which involves an a priori monolithic FSI formulation with the implicit detection of the fluid-structure interface and without limitations on the solid domain motion. The coupled weak forms of the fluid and structural mechanics equations are solved on the background mesh. Correspondence-based PD is used to model the meshfree solid in the foreground domain. We employ the Non-Uniform Rational B-Splines (NURBS) IGA functions in the background and the Reproducing Kernel Particle Method (RKPM) functions for the PD solid in the foreground. We feel that the combination of these numerical tools is particularly attractive for the problem class of interest due to the higher-order accuracy and smoothness of IGA and RKPM, the benefits of using immersed methodology in handling the fluid-structure coupling, and the capabilities of PD in simulating fracture and fragmentation scenarios. Numerical examples are provided to illustrate the performance of the proposed air-blast FSI framework.

==> PD_Body_Continuum.tex <==
%\documentclass[10pt]{article}
%\usepackage{pgf,tikz}
%\usepackage{mathrsfs}
%\usetikzlibrary{arrows}
%\pagestyle{empty}
%\begin{document}
\definecolor{wwqqzz}{rgb}{0.2,0.,0.8}
\resizebox {0.4\textwidth} {!} {
%\resizebox {5.8cm} {!} {
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
%\clip(0,0) rectangle (6.5,5.5);

% B 
\path (0,0.5) coordinate (A) (4,0) coordinate (B) (6,0.5) coordinate (C)(6.5,5.5) coordinate (D) (1,4.5) coordinate (E);
\draw[rounded corners=5mm, line width=1.4pt,fill=black,fill opacity=0.2] (A) -- (B) -- (C) -- (D) -- (E) -- cycle;
\draw (1.2,4.5) node[anchor=north west] {\large $\mathcal{B}$};

% H
\draw [line width=1.2pt,color=wwqqzz,fill=wwqqzz,fill opacity=0.2] (3.5,2.5) circle (2.1cm);
\draw (3.2,2.45) node[anchor=north west] {\large $\mathbf{x}$};
\draw [color=wwqqzz](2.3,1.4) node[anchor=north west] {\large $\mathcal{H}(\mathbf{x}) $};

% delta
\draw [->,>=stealth,line width=1.2pt,color=wwqqzz] (3.5,2.5) -- (5.2,3.7);
\draw [color=wwqqzz](3.9,3.7) node[anchor=north west] {\Large $\delta$};

% xi
\draw [->,>=stealth,line width=1.2pt,color=purple] (3.5,2.5) -- (2.6,3.2);
%\draw [color=purple](2.8,3.4) node[anchor=north west] {$\bs{\xi}$};

% x'
\draw (2,3.2) node[anchor=north west] {\large $\mathbf{x'}$};

% Points for x and x'
\begin{scriptsize}
\draw [fill=black] (3.5,2.5) circle (1.5pt);
\draw [fill=black] (2.57,3.2) circle (1.5pt);
\end{scriptsize}

\end{tikzpicture}
}
%\end{document}


==> PD_Body_Discrete.tex <==
%\documentclass[10pt]{article}
%\usepackage{pgf,tikz}
%\usepackage{mathrsfs}
%\usetikzlibrary{arrows}
%\pagestyle{empty}
%\begin{document}
\definecolor{wwqqzz}{rgb}{0.2,0.,0.8}
\resizebox {0.4\textwidth} {!} {
%\resizebox {5.8cm} {!} {
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=1.0cm,y=1.0cm]
%\clip(0,0) rectangle (6.5,5.5);

% B 
\path (0,0.5) coordinate (A) (4,0) coordinate (B) (6,0.5) coordinate (C)(6.5,5.5) coordinate (D) (1,4.5) coordinate (E);
\draw[rounded corners=5mm, line width=1.4pt,fill=white,fill opacity=0.2] (A) -- (B) -- (C) -- (D) -- (E) -- cycle;
\draw (1.3,4.5) node[anchor=north west] {\large $\tilde{\mathcal{B}}$};

% H
\draw [line width=1.2pt,color=wwqqzz,fill opacity=0.2] (3.85,2.5) circle (2.1cm);
\draw (3.6,2.45) node[anchor=north west] {\large $\mathbf{x}_I$};
\draw [color=wwqqzz](2.75,1.3) node[anchor=north west] {\large $\mathcal{H}_I$};

% delta
%\draw [->,>=stealth,line width=1.2pt,color=wwqqzz] (3.5,2.5) -- (4.8,3.3);
%\draw [color=wwqqzz](3.8,3.4) node[anchor=north west] {$\mathbf{\delta}$};

% xi
%\draw [->,>=stealth,line width=1.2pt,color=red] (3.5,2.5) -- (2.6,3);
%\draw [color=red](2.9,3.3) node[anchor=north west] {$\bs{\xi}_{ij}$};
\draw (2.55,2.4) node[anchor=north west] {\large $\mathbf{x}_J$};

% Points for x and x'
\begin{scriptsize}
\draw [fill=black] (0.6,0.85) circle (2pt);
\draw [fill=black] (1.6,0.7) circle (2pt);
\draw [fill=black] (2.6,0.6) circle (2pt);
\draw [fill=black] (3.6,0.5) circle (2pt);
\draw [fill=black] (4.6,0.65) circle (2pt);
\draw [fill=black] (5.5,0.85) circle (2pt);
\draw [fill=black] (5.65,1.8) circle (2pt);
\draw [fill=black] (5.75,2.8) circle (2pt);
\draw [fill=black] (5.85,3.85) circle (2pt);
\draw [fill=black] (5.95,4.9) circle (2pt);
\draw [fill=black] (5,4.75) circle (2pt);
\draw [fill=black] (4.05,4.6) circle (2pt);
\draw [fill=black] (3.1,4.45) circle (2pt);
\draw [fill=black] (2.15,4.3) circle (2pt);
\draw [fill=black] (1.25,4.15) circle (2pt);
\draw [fill=black] (1.1,3.3) circle (2pt);
\draw [fill=black] (0.9,2.45) circle (2pt);
\draw [fill=black] (0.75,1.65) circle (2pt);
\draw [fill=black] (1.75,1.55) circle (2pt);
\draw [fill=black] (2.75,1.45) circle (2pt);
\draw [fill=black] (3.75,1.35) circle (2pt);
\draw [fill=black] (4.75,1.45) circle (2pt);
\draw [fill=black] (4.85,2.6) circle (2pt);
\draw [fill=black] (4.95,3.75) circle (2pt);
\draw [fill=black] (3.95,3.65) circle (2pt);
\draw [fill=black] (2.95,3.55) circle (2pt);
\draw [fill=black] (1.95,3.45) circle (2pt);
\draw [fill=black] (1.85,2.45) circle (2pt);
\draw [fill=black] (2.85,2.45) circle (2pt);
\draw [fill=black] (3.85,2.5) circle (2pt);
\end{scriptsize}

\end{tikzpicture}
}
%\end{document}

